Optimizing Fitness-For-Use of Differentially Private Linear Queries

In practice, differentially private data releases are designed to support a variety of applications. A data release is fit for use if it meets target accuracy requirements for each application. In this paper, we consider the problem of answering linear queries under differential privacy subject to per-query accuracy constraints. Existing practical frameworks like the matrix mechanism do not provide such fine-grained control (they optimize total error, which allows some query answers to be more accurate than necessary, at the expense of other queries that become no longer useful). Thus, we design a fitness-for-use strategy that adds privacy-preserving Gaussian noise to query answers. The covariance structure of the noise is optimized to meet the fine-grained accuracy requirements while minimizing the cost to privacy.

==> analytical1.tex <==
\subsection{2-Dimensional Analytical Solution}
\addcolor{Suppose we have a 2-dimensional dataset} $\left[\begin{smallmatrix}x_1\\x_2\end{smallmatrix}\right]$ with a workload matrix $\mat{W}=\left[\begin{smallmatrix}1 & 1\\1 & 0\end{smallmatrix}\right]$ (i.e., the queries are $x_1+x_2$ and $x_1$). We want each query to be answered with Gaussian noise with variance at most 1 using the smallest possible privacy cost. The resulting mechanism\footnote{We set the basis matrix $\mat{B}=\mat{W}$.} is:
\begin{align*}
   \left[\begin{smallmatrix}1 & 1\\1 & 0\end{smallmatrix}\right] \left[\begin{smallmatrix}x_1\\x_2\end{smallmatrix}\right] + N\left(\vec{\mu}=\left[\begin{smallmatrix}0\\0\end{smallmatrix}\right], \mat{\Sigma}=\left[\begin{smallmatrix}a  & c\\c & d\end{smallmatrix}\right]\right) 
\end{align*}
and we need to optimize for \addcolor{ $a,c,d$}. The variances for the first and second workload queries are $a$ and $d$, respectively. The privacy cost $\Delta_M$ is $\sqrt{\max\left( [1, 1]\mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\1\end{smallmatrix}\right], ~ [1, 0] \mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\0\end{smallmatrix}\right]\right)}$.

\subsubsection{Sum-Squared Error Optimization}
Thus, the optimization problem for sum squared error given a fixed privacy cost $\beta$ is:
\begin{align}
    &\arg\min_{a,c,d} a + d\label{eqn:2dsum}\\
    &\text{ s.t. } a > 0, d> 0\nonumber\\
    &\text{ and } \Sigma\equiv\left[\begin{smallmatrix}a  & c\\c & d\end{smallmatrix}\right]\text{ is symmetric positive definite }\nonumber\\
    &\text{ and } \sqrt{\max\left( [1, 1]\mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\1\end{smallmatrix}\right], ~ [1, 0] \mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\0\end{smallmatrix}\right]\right)} \leq \beta\nonumber
\end{align}

\begin{textAtEnd}[category=section5]
We need the following technical result.
\end{textAtEnd}
\begin{theoremEnd}[category=section5,all end]{lemma}\label{lemma:helpful}
Let $a>d>0$. Then $ad < (a-\gamma)(d+\gamma)$ when $\gamma < (a-d)/2$.
\end{theoremEnd}
\begin{proofEnd}
We need to show that $ad - (a-\gamma)(d+\gamma)= d\gamma -a\gamma + \gamma^2 < 0$.  Taking derivatives with respect to $\gamma$, we get
\begin{align*}
    \frac{\partial (d\gamma -a\gamma + \gamma^2)}{\partial \gamma} &= d-a+2\gamma
\end{align*}
The derivative is negative if and only if $\gamma < (a-d)/2$. The result follows by noting that $ad - (a-\gamma)(d+\gamma)= d\gamma -a\gamma + \gamma^2 $ equals $0$ at $\gamma=0$.
\end{proofEnd}

\begin{theoremEnd}[category=section5]{theorem}\label{thm:eqn:2dsum} The solution to the optimization problem in Equation \ref{eqn:2dsum} is  $a= \frac{1 + \frac{1}{\sqrt{5}}}{\beta^2}$, $d=\frac{\frac{1}{2}+\frac{3}{10}\sqrt{5}}{\beta^2}$, $c=\frac{1 + \frac{1}{\sqrt{5}}}{2\beta^2}$ (so $\mat{\Sigma}\approx\frac{1}{\beta^2}\left[\begin{smallmatrix}1.45, & 0.72\\ 0.72, & 1.17\end{smallmatrix}\right]$), which achieves an objective function value of $\frac{\frac{3}{2} + \frac{\sqrt{5}}{2}}{\beta^2}$.
\end{theoremEnd}
\begin{proofEnd}
Note that for $\mat{\Sigma}$ to be symmetric positive definite, the eigenvalues must be positive. In two dimensions, this is the same as requiring (1) the trace (sum along the diagonal, which is equal to the sum of the eigenvalues) to be positive and (2) the determinant (which is equal to the product of the eigenvalues) to be positive. Thus we must have
\begin{align*}
    a &> 0\\
    d &> 0\\
    ad-c^2 &>0
\end{align*}
We also note that the 
\begin{align*}
    \mat{\Sigma}^{-1} &=\frac{1}{ad-c^2}\left[\begin{smallmatrix}d  & -c\\-c & a\end{smallmatrix}\right]
\end{align*}
So that the privacy cost is:
\begin{align*}
    &\sqrt{\max\left( [1, 1]\mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\1\end{smallmatrix}\right], [1, 0] \mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\0\end{smallmatrix}\right]\right)}  \\
    &= \sqrt{\max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right)} 
\end{align*}
and the optimization problem simplifies to:
\begin{align}
    &\arg\min_{a,c,d} a+d\label{eq:proofsum1}\\
    &\text{ s. t. } a > 0, d > 0\nonumber\\
    &\text{ and } ad-c^2 >0\nonumber\\
    &\text{ and } \max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right)\leq \beta^2\nonumber
\end{align}

We first derive a sequence of facts about solutions to this problem:

\vspace{0.5em}
\noindent\textbf{\underline{Fact 0}: if $\max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right) < \beta^2$ then $a+d$ is larger than the optimal objective function value.} By way of contradiction, assume $a^*, d^*, c^*$ was an optimal solution and that the quantity $\max\left( \frac{a^*+d^*-2c^*}{a^*d^*-(c^*)^2}, \frac{d^*}{a^*d^*-(c^*)^2}\right)<\beta^2$. If $\gamma>1$ then consider setting $a=a^*/\gamma, d=d^*/\gamma, c=c^*/\gamma$. Clearly, $a+d< a^*+d^*$ (decreasing the objective function) while $\max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right)= \gamma \max\left( \frac{a^*+d^*-2c^*}{a^*d^*-(c^*)^2}, \frac{d^*}{a^*d^*-(c^*)^2}\right)$. If $\gamma>1$ but close enough to $1$ then $\max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right)\leq \beta^2$, which shows that $a,d,c$ satisfies the constraints and lowers the objective function, contradicting the optimality of  $a^*, d^*, c^*$.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 1}: $\frac{d}{ad-c^2}$ is (1a) decreasing in $d$, (1b) decreasing in $a$, (1c) increasing in $c$ over the region where $ad > c^2$ and $a>0$ and $d>0$ and $c\geq 0$.} This is obvious for (1b) and (1c). For (1a), we can see this from $\frac{d}{ad-c^2}=\frac{1}{a-c^2/d}$. 
    
\vspace{0.5em}
\noindent\textbf{\underline{Fact 2}: $a+d>2c$ when $ad>c^2$ and $c\geq 0$ and $a>0$ and $d>0$}. This is true because $\Sigma^{-1}$ is symmetric positive definite under these conditions (see the very first two sentences of the proof) and $a+d-2c$ is a positive multiple of the positive quantity $[1, 1]\Sigma^{-1}\left[\begin{smallmatrix}1 \\ 1\end{smallmatrix}\right]$ (this quantity is positive because of positive definiteness and the positive multiple is $ad-c^2$, which is positive under this conditions).

\vspace{0.5em}
\noindent\textbf{\underline{Fact 3}: $\frac{a+d-2c}{ad-c^2}$ is decreasing in $a$ and $d$ over the region  where $ad > c^2$ and $a>0$ and $d>0$ and $c\geq 0$}. For $d$, this can be shown by taking the log and then checking if the derivative is negative. $\frac{\partial}{\partial d}\log \frac{a+d-2c}{ad-c^2} = \frac{1}{a+d-2c} - \frac{a}{ad-c^2} = \frac{ad-c^2 - a(a+d-2c)}{(a+d-2c)(ad-c^2)}=-\frac{(a-c)^2}{(a+d-2c)(ad-c^2)}$. This quantity is negative because the numerator is positive, the first term in the denominator is positive (from Fact 2) and the second term in the denominator is positive in the region considered by the current fact (i.e., Fact 3). By symmetry, $\frac{a+d-2c}{ad-c^2}$ is decreasing in $a$ as well.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 4}: $\frac{a+d-2c}{ad-c^2}$ is increasing in $c$  if $c$ is between $a$ and $d$ and is decreasing otherwise ($c=a$ and $c=d$ are local extrema) over the region where $ad > c^2$ and $a>0$ and $d>0$ and $c\geq 0$}. This can be seen by taking the log and checking the sign of the derivative. $\frac{\partial}{\partial c}\log \frac{a+d-2c}{ad-c^2} = \frac{-2}{a+d-2c} - \frac{-2c}{ad-c^2}= \frac{-2(ad-c^2) + 2c(a+d-2c)}{(a+d-2c)(ad-c^2)}=\frac{2ac + 2cd - 2ad-2c^2}{(a+d-2c)(ad-c^2)}=-2\frac{(c-a)(c-d)}{(a+d-2c)(ad-c^2)}$. This derivative is positive if and only if $c$ is between $a$ and $d$, since the first term in the denominator is positive by Fact 2 and the second term in the denominator is positive in the region considered by the current Fact (i.e., Fact 4).


\vspace{0.5em}
\noindent\textbf{\underline{Fact 5}: if $a^*, d^*, c^*$ is optimal and $c^*<0$ then $a=a^*, d=d^*, c=|c^*|$ and hence we can assume $c\geq 0$.} Clearly all of the constraints remain feasible and the objective function remains unchanged.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 6}: if $a^*, d^*, c^*$ is optimal, then $d^*\leq a^*$.}  To see why, suppose by way of contradiction that  $d^*>a^*$. If that happens, we can create a new solution with $d_1=a^*$, $a_1=d^*$ and $c_1=c^*$. Then $d^*=a_1  > d_1$ and so $\beta^2 \geq \frac{d^*}{a^*d^*-(c^*)^2} > \frac{d_1}{a_1d_1-c_1^2}$. Clearly $a_1,d_1,c_1$ satisfy the constraints of the optimization problem in Eq \ref{eq:proofsum1} and give the same value for the objective function as the optimal solution $d^*,a^*,c^*$ did. Now, choose a $\gamma\in (0, (a_1-d_1)/2)$ that is small enough so that we still have $\beta^2 > \frac{d_1+\gamma}{(a_1-\gamma)(d_1+\gamma)-c_1^2}$. Then set $a_2 =a_1-\gamma, d_2 = d_1+\gamma, c_2=c_1$. Then, by Lemma \ref{lemma:helpful}, we have $\beta^2\geq \frac{a^*+d^*-2c^*}{a^*d^*-(c^*)^2}=\frac{a_1+d_1-2c_1}{a_1d_1-c_1^2} > \frac{a_2+d_2-2c_2}{a_2d_2-c_2^2}$. So we have shown that $\max\left( \frac{a_2+d_2-2c_2}{a_2d_2-c_2^2}, \frac{d_2}{a_2d_2-c_2^2}\right) < \beta^2$. Meanwhile, $a_2+d_2=a_1+d_1=a^*+d^*$ so, by Fact 0, $a^*,d^*,c^*$ cannot be optimal.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 7}: if $a^*, d^*, c^*$ is optimal and $c^*>d^*$ then there exists an optimal solution with $a=a^*, d=d^*, c\in [0,d]$.}
Note that the variable $c^*$ is not part of the objective function and is only involved in the constrains $a^*d^*-(c^*)^2>0$ and $\max\left( \frac{a^*+d^*-2c^*}{a^*d^*-(c^*)^2}, \frac{d^*}{a^*d^*-(c^*)^2}\right)\leq \beta^2$. Lowering the value of $c^*$ keeps the constraint $a^*d^*-(c^*)^2>0$ feasible. We note that $c* < a^*$ (otherwise $a^*d^*-(c^*)^2\leq 0$, as $a^*\geq d^*$ by Fact 6). If $d^*<c^* < a^*$ then by Facts 1 and 4, we can decrease $c^*$ until it reaches $d^*$ while at the same time reducing $\max\left( \frac{a^*+d^*-2c^*}{a^*d^*-(c^*)^2}, \frac{d^*}{a^*d^*-(c^*)^2}\right)$ and so the constraints remain feasible.

\vspace{0.5em}
Thus, by Facts 5,and 7 there are 3 cases to consider: $c=0$, $c=d$, and $0<c<d$. For each of these cases, we will find the best choice of $a$ and $d$, and then we will compare these cases to find which one results in a smaller objective function value (i.e., $a+d$).

\vspace{0.5cm}
\noindent\textbf{Case 1: $c=0$.}
In this case, the problem reduces to $\arg\min\limits_{a,d} a+d $ s.t. $a>0, d>0$ and $\max(\frac{a+d}{ad}, \frac{1}{a}) \leq \beta^2$. Now, since $\frac{a+d}{ad}\leq\beta^2$, we must have $1 < a\beta^2$ (otherwise $(a+d)/(ad)\leq \beta^2\Rightarrow a+d \leq d(a\beta^2)\leq d$ which is impossible). For similar reasons, $1 < d\beta^2$. Now, if you fix the sum $b=a+d$, then the fraction $\frac{a+d}{ad}$ is smallest when $a=d=b/2$ so the problem simplifies to $\arg\min\limits_{a} 2a$ s.t., $a>0$ and $2/a\leq \beta^2$ which is optimized by setting $a=2/\beta^2$. To summarize, analysis of Case 1 results in the following candidate solution: \underline{$a=2/\beta^2$, $d=2/\beta^2$, $c=0$} with objective value \underline{$4/\beta^2$}.


\vspace{0.5cm}
\noindent\textbf{Case 2: $c=d$.}
In this case the problem simplifies to $\arg\min\limits_{a,d} a+d$ s.t., $a > 0, d>0$ and $\max(\frac{a-d}{d(a-d)}, \frac{d}{d(a-d)}) = \max(\frac{1}{d}, \frac{1}{(a-d)})\leq \beta^2$. For any $d$, from the last inequality, we see that $1\leq (a-d)\beta^2$ and so the best choice of $a$ is $d + 1/\beta^2$. The problem simplifies to $\arg\min\limits_{d} 2d+1/\beta^2$ s.t., $d>0$ and $1/d\leq\beta^2$. Clearly the optimal choice is $d=1/\beta^2$. Thus, we get a candidate solution of \underline{$a=2/\beta^2, d=1/\beta^2, c=1/\beta^2$} with objective value \underline{$3/\beta^2$}.

\vspace{0.5cm}
\noindent\textbf{Case 3: $0 < c < d$.} By Facts 1 and 4, increasing $c$ slightly will decrease $\frac{a+d-2c}{ad-c^2}$ and increase $\frac{d}{ad-c^2}$ while decreasing $c$ will have the opposite effect. Thus, we must have $\frac{a+d-2c}{ad-c^2}=\beta^2=\frac{d}{ad-c^2}$. Otherwise, if $\beta^2$ is strictly larger than one of these terms, we can adjust $c$ so that both terms are strictly smaller than $\beta^2$ (and by Fact 0, the values of $a$ and $d$ would not be optimal). Now, $\frac{a+d-2c}{ad-c^2}=\beta^2=\frac{d}{ad-c^2}$ implies $a=2c$ so from Fact 6 we have $d\leq a=2c < 2d$. Thus the problem simplifies to $\arg\min\limits_{a,d} a+d$ s.t. $0<d\leq a<2d$ and $\frac{d}{ad-a^2/4}=\beta^2$. Then we solve for $d$ in terms of $a$:

\begin{align*}
\frac{d}{ad-a^2/4}=\beta^2 &\Leftrightarrow a^2\beta^2/4 = d a \beta^2 - d\\
&\Leftrightarrow d = \frac{a^2\beta^2}{4(a\beta^2-1)} = \frac{a}{4} + \frac{a}{4(a\beta^2-1)}
\end{align*}
and the problem simplifies to $\arg\min\limits_a \frac{5a}{4} + \frac{a}{4(a\beta^2-1)}$ s.t., $0 < \frac{a}{4} + \frac{a}{4(a\beta^2-1)} \leq a < 2\left(\frac{a}{4} + \frac{a}{4(a\beta^2-1)}\right)$.
and so if an optimal solution exists in Case 3, then it is either at a place where the derivative of the objective function is 0 or at the boundary $a= \frac{a}{4} + \frac{a}{4(a\beta^2-1)}$. If it occurs at the boundary, then we get \underline{$a=\frac{4}{3\beta^2}=d$ and $c=\frac{2}{3\beta^2}$} for an objective function value of \underline{$\frac{8}{3\beta^2}$}. On the other hand, if we look at the extremum, we see:
\begin{align*}
    \frac{\partial ( \frac{5a}{4} + \frac{a}{4(a\beta^2-1)})}{\partial a} &= \frac{5}{4} + \frac{a\beta^2-1 - a\beta^2}{4(a\beta^2-1)^2} = \frac{5}{4} - \frac{1}{4(a\beta^2-1)^2}
\end{align*}
which is $0$ at the point $a = (1 + \frac{1}{\sqrt{5}})/\beta^2$. Then 
\begin{align*}
    d &= \frac{a}{4} + \frac{a}{4(a\beta^2-1)} = \frac{(1 + 1/{\sqrt{5}})}{4\beta^2} + \frac{(1 + 1/\sqrt{5})/\beta^2}{4/\sqrt{5}}\\
      &= \frac{\frac{1}{2}+\frac{3}{10}\sqrt{5}}{\beta^2}
\end{align*}
Thus the other candidate is \underline{$a= (1 + \frac{1}{\sqrt{5}})/\beta^2$},\underline{ $d=\frac{\frac{1}{2}+\frac{3}{10}\sqrt{5}}{\beta^2}$}, \underline{$c=\frac{(1 + \frac{1}{\sqrt{5}})}{2\beta^2}$} for an objective function value of \underline{$\frac{\frac{3}{2} + \frac{\sqrt{5}}{{2}}}{\beta^2}$}. It is straightforward to check that this is a feasible solution to the optimization problem in Equation \ref{eq:proofsum1}.

Comparing the 4 solutions (2 from Case 3 and 1 each from Cases 1 and 2), we see that the smallest objective function is obtained when  $a= (1 + \frac{1}{\sqrt{5}})/\beta^2$, $d=\frac{\frac{1}{2}+\frac{3}{10}\sqrt{5}}{\beta^2}$, $c=\frac{(1 + \frac{1}{\sqrt{5}})}{2\beta^2}$.
\end{proofEnd}

Thus we see that if we desire a privacy level of $\Delta_M=\beta$, the variance of the first query is $(1+1/\sqrt{5})/\beta^2\approx 1.45/\beta^2$ and for the second query it is $\approx 1.17/\beta^2$. The queries ended up having different variances even though they were weighted the same (i.e., the objective function is the sum of their variances, with no preference given between the two queries).

\subsubsection{Fitness-for-use Optimization}
We can optimize for fitness for use instead by directly solving Problem \ref{problem1} for this example, setting the target variances for the two queries to be a most some number $\gamma$. The optimization problem reduces to:

\begin{align}
    & \arg\min_{a,c,d} \max\left( [1, 1]\mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\1\end{smallmatrix}\right], ~ [1, 0] \mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\0\end{smallmatrix}\right]\right)\label{eqn:2dfit}\\
    &\text{ s.t. } \Sigma\equiv\left[\begin{smallmatrix}a  & c\\c & d\end{smallmatrix}\right]\text{ is positive definite }\nonumber\\
    &\text{ and } a\leq \gamma, d\leq \gamma \nonumber
\end{align}

\begin{theoremEnd}[category=section5]{theorem}\label{thm:eqn:2dfit} The solution to Equation \ref{eqn:2dfit} is  $a=d=\gamma$ and $c=\gamma/2$ (so $\mat{\Sigma}=\gamma\left[\begin{smallmatrix}1, & 0.5\\0.5, & 1\end{smallmatrix}\right]$), which achieves a privacy cost of $\sqrt{\frac{4}{3\gamma}}$.
\end{theoremEnd}
\begin{proofEnd}
Note that for $\mat{\Sigma}$ to be symmetric positive definite, the eigenvalues must be positive. In two dimensions, this is the same as requiring (1) the trace (sum along the diagonal, which is equal to the sum of the eigenvalues) to be positive and (2) the determinant (which is equal to the product of the eigenvalues) to be positive. Thus we must have
\begin{align*}
    a &> 0\\
    d &> 0\\
    ad-c^2 &>0
\end{align*}
We also note that the 
\begin{align*}
    \mat{\Sigma}^{-1} &=\frac{1}{ad-c^2}\left[\begin{smallmatrix}d  & -c\\-c & a\end{smallmatrix}\right]
\end{align*}
So that the privacy cost is:
\begin{align*}
    &\sqrt{\max\left( [1, 1]\mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\1\end{smallmatrix}\right], ~ [1, 0] \mat{\Sigma}^{-1} \left[\begin{smallmatrix}1\\0\end{smallmatrix}\right]\right)} \\
    = &\sqrt{\max\left( \frac{a+d-2c}{ad-c^2}, \frac{d}{ad-c^2}\right)} 
\end{align*}
and the optimization problem simplifies to:
\begin{align}
&\arg\min_{a,c,d} \max\left(\frac{d}{ad-c^2}, \frac{a+d-2c}{ad-c^2}\right) \label{eqn:prooffit}\\
&\text{ s.t. } a\leq \gamma, d\leq \gamma\nonumber\\
&\text{ and } ad-c^2 > 0\nonumber
\end{align}

We will prove the result through a series of facts.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 0}: If $a^*, d^*, c^*$ is an optimal solution, so is $a=a^*, d=d^*, c=|c^*|$ so we can assume $c\geq 0$.} This is obvious from the objective function and constraints.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 1}: $\frac{d}{ad-c^2}$ is (1a) decreasing in $d$, (1b) decreasing in $a$ over the region where $ad > c^2$ and $a>0$ and $d>0$ and $c\geq 0$.} This is obvious for (1b). For (1a), we can see this from $\frac{d}{ad-c^2}=\frac{1}{a-c^2/d}$. 
    
\vspace{0.5em}
\noindent\textbf{\underline{Fact 2}: $a+d>2c$ when $ad>c^2$ and $c\geq 0$ and $a>0$ and $d>0$}. This is true because $\Sigma^{-1}$ is positive definite under these conditions (see the very first two sentences of the proof) and $a+d-2c$ is a positive multiple of the positive quantity $[1, 1]\Sigma^{-1}\left[\begin{smallmatrix}1 \\ 1\end{smallmatrix}\right]$ (this quantity is positive because of positive definiteness and the positive multiple is $ad-c^2$, which is positive under this conditions).

\vspace{0.5em}
\noindent\textbf{\underline{Fact 3}: $\frac{a+d-2c}{ad-c^2}$ is decreasing in $a$ and $d$ over the region  where $ad > c^2$ and $a>0$ and $d>0$ and $c\geq 0$}. For $d$, this can be shown by taking the log and then checking if the derivative is negative. $\frac{\partial}{\partial d}\log \frac{a+d-2c}{ad-c^2} = \frac{1}{a+d-2c} - \frac{a}{ad-c^2} = \frac{ad-c^2 - a(a+d-2c)}{(a+d-2c)(ad-c^2)}=-\frac{(a-c)^2}{(a+d-2c)(ad-c^2)}$. This quantity is negative because the numerator is positive, the first term in the denominator is positive (from Fact 2) and the second term in the denominator is positive in the region considered by the current (i.e., Fact 3). By symmetry, $\frac{a+d-2c}{ad-c^2}$ is decreasing in $a$ as well.

\vspace{0.5em}
\noindent\textbf{\underline{Fact 4}: In the optimal solution, $a =\gamma$ and $d=\gamma$.} If $a<\gamma$, then we can increase $a$ while decreasing the objective function (Facts 1 and 3), and similarly for $d$.

\vspace{0.5em}
\noindent Fact 4 simplifies the objective function to minimizing \\$ \max\left(\frac{\gamma}{\gamma^2-c^2}, \frac{2\gamma-2c}{\gamma^2-c^2}\right)$. Note that $\frac{2\gamma-2c}{\gamma^2-c^2}=\frac{2}{\gamma+c}$, so the problem simplifies to

\begin{align}
&\arg\min_{c} \max\left(\frac{\gamma}{\gamma^2-c^2}, \frac{2}{\gamma+c}\right) \label{eqn:prooffit:b}\\
&\text{ s.t. }  \gamma^2-c^2 > 0\nonumber
\end{align}

 Note that the first term in the objective function in Equation \ref{eqn:prooffit:b} is increasing in $c$ while the second is decreasing at $c$. Therefore the minimum occurs either at the boundary point $c=0$  or when the two terms are equal. If $c=0$ then the objective function value is $2/\gamma$. 
 
 If the two terms in the objective function are equal then: 
 \begin{align*}
   &\frac{\gamma}{\gamma^2-c^2}= \frac{2}{\gamma+c}\\
& \Leftrightarrow \frac{\gamma}{\gamma-c}= 2\\
& \Leftrightarrow \gamma = 2\gamma - 2c\\
& \Leftrightarrow c=\gamma/2
 \end{align*}
 In this case, the value of the objective function is $4/(3\gamma)$ (which is lower than in the case $c=0$, and we take the square root to get the privacy cost). Thus the optimal solution is $a=d=\gamma$ and $c=\gamma/2$.

\end{proofEnd}

We can compare both theorems by forcing both mechanisms to have the same privacy cost (e.g., set $\gamma=1$ and $\beta=\sqrt{4/(3\gamma)}$). In this case, the fitness-for-use optimization answers both queries with variance $1$, but the sum-squared optimization results in a maximum per-query variance of $1.08$. The difference is small in this 2-dimensional toy problem but can be substantial in larger workloads (see experiments in Section \ref{sec:experiments}). 

The main take-home message is that sum-squared optimization and fitness-for-use optimization produce very different solutions, and only fitness-for-use optimization allows us to carefully tune the desired variance for each query answer.


==> notes2.tex <==
\subsection{Original Problem}
\begin{theorem}
Suppose $\mat{W} = \mat{W}_1 \otimes \mat{W}_2$, $\vec{c}  = \vec{c}_2 \otimes \vec{c}_1$
\begin{align}
    \alpha_1,\mat{\Sigma}_1 & \leftarrow \arg\min_{\mat{\alpha_1,\mat{\Sigma}_1}} \alpha_1 \\
     & \phantom{\leftarrow}\text{s.t. } \vec{b}_{1i}^T\mat{\Sigma}_1^{-1}\vec{b}_{1i}\leq \alpha_1 \text{ for all $i=1,\dots, d$}\nonumber\\
     & \phantom{\leftarrow}\text{and } \vec{v}_{1j}\mat{\Sigma_1} \vec{v}_{1j}^T \leq c_{1j} \text{ for $j=1,\dots, m$}\nonumber\\
     & \phantom{\leftarrow}\text{and $\mat{\Sigma}_1$ is symmetric positive definite.}\nonumber
\end{align}

\begin{align}
    \alpha_2,\mat{\Sigma}_2 & \leftarrow \arg\min_{\mat{\alpha_2,\mat{\Sigma}_2}} \alpha_2 \\
     & \phantom{\leftarrow}\text{s.t. } \vec{b}_{2i}^T\mat{\Sigma}_2^{-1}\vec{b}_{2i}\leq \alpha_2 \text{ for all $i=1,\dots, d$}\nonumber\\
     & \phantom{\leftarrow}\text{and } \vec{v}_{2j}\mat{\Sigma_2} \vec{v}_{2j}^T \leq c_{2j} \text{ for $j=1,\dots, m$}\nonumber\\
     & \phantom{\leftarrow}\text{and $\mat{\Sigma}_2$ is symmetric positive definite.}\nonumber
\end{align}

Let 
\begin{align*}
    \mat{\Sigma} &= \mat{\Sigma}_1 \otimes \mat{\Sigma}_2 \\
    \alpha &= \alpha_1 * \alpha_2 \\
    \mat{B} &= \mat{B}_1 \otimes \mat{B}_2 \\
    \mat{L} &= \mat{L}_1 \otimes \mat{L}_2
\end{align*}
so that
\begin{align*}
    \vec{b}_i &= \vec{b}_{1i} \otimes \vec{b}_{2i} \\
    \vec{v}_j &= \vec{v}_{1j} \otimes \vec{v}_{2j} \\
    \mat{W} &= \left( \mat{L}_1 \otimes \mat{L}_2 \right) \left( \mat{B}_1 \otimes \mat{B}_2 \right) \\
    &= \mat{L}_1 \mat{B}_1 \otimes \mat{L}_2 \mat{B}_2 \\
    &= \mat{W}_1 \otimes \mat{W}_2
\end{align*}
Then we have
\begin{align}
     &pcost = \max_i \vec{b}_{i}^T\mat{\Sigma}^{-1}\vec{b}_{i} \leq \alpha \\
     & \phantom{\leftarrow}\text{s.t. } \vec{b}_{i}^T\mat{\Sigma}^{-1}\vec{b}_{i}\leq \alpha \text{ for all $i=1,\dots, d$}\nonumber\\
     & \phantom{\leftarrow}\text{and } \vec{v}_{j}\mat{\Sigma} \vec{v}_{j}^T \leq c_{j} \text{ for $j=1,\dots, m$}\nonumber\\
     & \phantom{\leftarrow}\text{and $\mat{\Sigma}$ is symmetric positive definite.}\nonumber
\end{align}

\end{theorem}

\begin{proof}
Firstly
\begin{align*}
    &\quad \vec{b}_{i}^T\mat{\Sigma}^{-1}\vec{b}_{i} \\
    &= (\vec{b}_{1i} \otimes \vec{b}_{2i} ) (\mat{\Sigma}_1 \otimes \mat{\Sigma}_2 )^{-1} ( \vec{b}_{1i} \otimes \vec{b}_{2i}) \\
    &= (\vec{b}_{1i}^T \otimes \vec{b}_{2i}^T ) (\mat{\Sigma}_1^{-1} \otimes \mat{\Sigma}_2^{-1} ) ( \vec{b}_{1i} \otimes \vec{b}_{2i}) \\ 
    &= (\vec{b}_{1i}^T \mat{\Sigma}_1 \otimes \vec{b}_{2i}^T \mat{\Sigma}_2 ) ( \vec{b}_{1i} \otimes \vec{b}_{2i}) \\
    &= (\vec{b}_{1i}^T \mat{\Sigma}_1 \vec{b}_{1i} \otimes \vec{b}_{2i}^T \mat{\Sigma}_2 \vec{b}_{2i} ) \\
    &\leq  \alpha_1 * \alpha_2 \\
    &= \alpha
\end{align*}
Secondly
\begin{align*}
    &\quad \vec{v}_{j}\mat{\Sigma}\vec{v}_{j}^T \\
    &= (\vec{v}_{1j} \otimes \vec{v}_{2j} ) (\mat{\Sigma}_1 \otimes \mat{\Sigma}_2 ) ( \vec{v}_{1j} \otimes \vec{v}_{2j})^T \\
    &= (\vec{v}_{1j} \mat{\Sigma}_1 \otimes \vec{v}_{2j} \mat{\Sigma}_2)  ( \vec{v}_{1j}^T \otimes \vec{v}_{2j}^T) \\
    &=(\vec{v}_{1j} \mat{\Sigma}_1  \vec{v}_{1j}^T \otimes \vec{v}_{2j} \mat{\Sigma}_2 \vec{v}_{2j}^T)  \\
    &\leq \vec{c}_{1j} \otimes \vec{c}_{2j} \\
    &= \vec{c}_{1j} * \vec{c}_{2j} \\
    &= \vec{c}_j
\end{align*}
Lastly, because $\mat{\Sigma}_1$, $\mat{\Sigma}_2$ are both positive definite, $\mat{\Sigma} = \mat{\Sigma}_1 \otimes \mat{\Sigma}_2 $ is also positive definite.
\end{proof}

\subsection{SM-II Problem}
\begin{align}
     \mat{\Sigma}^* & \leftarrow \arg\min_{\mat{\Sigma}} \frac{1}{t_1}\log\left(\sum_i \exp(t_1*\vec{b}_i^T\mat{\Sigma}^{-1}\vec{b}_i)\right)\\
    &\phantom{\leftarrow \arg\min_{\mat{\Sigma}}} + \frac{1}{t_2}\log\left(\sum_j t_2*\frac{\vec{v}_j \mat{\Sigma} \vec{v}_j^T}{c_j}\right) \nonumber\\
     & \phantom{\leftarrow}\text{s.t. $\mat{\Sigma}$ is symmetric positive definite.}\nonumber
\end{align}
Suppose we have $\mat{W} = \mat{W}_1 \otimes \mat{W}_2$, $\mat{\Sigma} = \mat{\Sigma}_1 \otimes \mat{\Sigma}_2$, we can get $\mat{\Sigma}_1$, $\mat{\Sigma}_2$ by cyclically updating their values.

\begin{align}
     \mat{\Sigma}_1 & \leftarrow \arg\min_{\mat{\Sigma}_1} \frac{1}{t_1}\log\left(\sum_i \exp(t_1*\vec{b}_{1i}^T\mat{\Sigma}_1^{-1}\vec{b}_{1i} * \vec{b}_{2i}^T\mat{\Sigma}_2^{-1}\vec{b}_{2i})\right)\\
    &\phantom{\leftarrow \arg\min_{\mat{\Sigma}_2}} + \frac{1}{t_2}\log\left(\sum_j \frac{t_2}{c_j} * \vec{v}_{1j} \mat{\Sigma}_1 \vec{v}_{1j}^T * \vec{v}_{2j} \mat{\Sigma}_2 \vec{v}_{2j}^T\right) \nonumber\\
     & \phantom{\leftarrow}\text{s.t. $\mat{\Sigma}_1$ is symmetric positive definite, $\mat{\Sigma}_2$ is fixed.}\nonumber
\end{align}

\begin{align}
     \mat{\Sigma}_2 & \leftarrow \arg\min_{\mat{\Sigma}_2} \frac{1}{t_1}\log\left(\sum_i \exp(t_1*\vec{b}_{1i}^T\mat{\Sigma}_1^{-1}\vec{b}_{1i} * \vec{b}_{2i}^T\mat{\Sigma}_2^{-1}\vec{b}_{2i})\right)\\
    &\phantom{\leftarrow \arg\min_{\mat{\Sigma}_2}} + \frac{1}{t_2}\log\left(\sum_j \frac{t_2}{c_j} * \vec{v}_{1j} \mat{\Sigma}_1 \vec{v}_{1j}^T * \vec{v}_{2j} \mat{\Sigma}_2 \vec{v}_{2j}^T\right) \nonumber\\
     & \phantom{\leftarrow}\text{s.t. $\mat{\Sigma}_2$ is symmetric positive definite, $\mat{\Sigma}_1$ is fixed.}\nonumber
\end{align}

\newpage

\subsection{Weighted Combination}
\begin{align}
    \mat{W}=
    \begin{bmatrix}
        \mat{W}_a  \\
        \mat{W}_b  
    \end{bmatrix}
\end{align}

Where $\mat{W}_a = \mat{W}_1 \otimes \mat{W}_2$, $\mat{W}_b = \mat{W}_3 \otimes \mat{W}_4$.

Given privacy constraints$\vec{c}_a$, $\vec{c}_b$, We use previous algorithm to get $\mat{\Sigma}_a$, $\mat{\Sigma}_b$.

Can we use a weighted combination of $\mat{\Sigma}_a$ and $\mat{\Sigma}_b$ to approximate the optimal solution $\mat{\Sigma}^{\star}$? That is, $\mat{\Sigma}=t_a\mat{\Sigma}_a + t_b \mat{\Sigma}_b$

\begin{align}
    t_a, t_b & \leftarrow \arg\min_{t_a, t_b} \alpha \\
     & \phantom{\leftarrow}\text{s.t. } \vec{b}_i^T\mat{\Sigma}^{-1}\vec{b}_{i}\leq \alpha \text{ for all $i=1,\dots, d$}\nonumber\\
     & \phantom{\leftarrow}\text{and } \vec{v}_{j}\mat{\Sigma} \vec{v}_{j}^T \leq c_{j} \text{ for $j=1,\dots, m$}\nonumber\\
     & \phantom{\leftarrow}\text{and $\mat{\Sigma}=t_a\mat{\Sigma}_a + t_b \mat{\Sigma}_b$ is symmetric positive definite.}\nonumber
     \label{prob:t}
\end{align}

% The intuition is that, given 
% \begin{align*}
%     &\vec{v}_{j}\mat{\Sigma}_a \vec{v}_{j}^T \leq c_{j} \text{ for $j=1,\dots, m_a$} \\
%     &\vec{v}_{j}\mat{\Sigma}_b \vec{v}_{j}^T \leq c_{j} \text{ for $j=m_a+1,\dots, m_a+m_b$}
% \end{align*}
% We can find a weighted combination of $\mat{\Sigma}_a$ and $\mat{\Sigma}_b$, that is $\mat{\Sigma}=t_a\mat{\Sigma}_a + t_b \mat{\Sigma}_b$, which satisfies
% \begin{align*}
%     &\vec{v}_{j} (t_a\mat{\Sigma}_a + t_b \mat{\Sigma}_b) \vec{v}_{j}^T \leq c_{j} \text{ for $j=1,\dots, m_a+m_b$} 
% \end{align*}

Because the function $f(\mat{\Sigma}) = \mat{\Sigma}^{-1}$ is matrix convex, we have 
\begin{align}
    &(t_a\mat{\Sigma}_a + t_b \mat{\Sigma}_b)^{-1} \leq t_a \mat{\Sigma}_a^{-1} + t_b \mat{\Sigma}_b^{-1}\\ &t_a + t_b = 1, t_a \ge 0, t_b \ge 0
\end{align}

So that we can approximate the problem \ref{prob:t} 
\begin{align}
    t_a, t_b & \leftarrow \arg\min_{t_a, t_b} \alpha \\
     & \phantom{\leftarrow}\text{s.t. } t_a\vec{b}_i^T\mat{\Sigma}_a^{-1}\vec{b}_{i} + t_b \vec{b}_i^T\mat{\Sigma}_a^{-1}\vec{b}_{i} \leq \alpha \text{ for all $i=1,\dots, d$}\nonumber\\
     & \phantom{\leftarrow}\text{and } t_a\vec{v}_{j}\mat{\Sigma}_a \vec{v}_{j}^T + t_b\vec{v}_{j}\mat{\Sigma}_b \vec{v}_{j}^T \leq c_{j} \text{ for $j=1,\dots, m$}\nonumber\\
     & \phantom{\leftarrow}\text{and $t_a + t_b =1, t_a \geq 0, t_b \geq 0$ }\nonumber
\end{align}
